Equitable Restless Multi-Armed Bandits: A General Framework Inspired By Digital Health

Restless multi-armed bandits (RMABs) are a popular framework for algorithmic decision making in sequential settings with limited resources. RMABs are increasingly being used for sensitive decisions such as in public health, treatment scheduling, anti-poaching, and -- the motivation for this work -- digital health. For such high stakes settings, decisions must both improve outcomes and prevent disparities between groups (e.g., ensure health equity). We study equitable objectives for RMABs (ERMABs) for the first time. We consider two equity-aligned objectives from the fairness literature, minimax reward and max Nash welfare. We develop efficient algorithms for solving each -- a water filling algorithm for the former, and a greedy algorithm with theoretically motivated nuance to balance disparate group sizes for the latter. Finally, we demonstrate across three simulation domains, including a new digital health model, that our approaches can be multiple times more equitable than the current state of the art without drastic sacrifices to utility. Our findings underscore our work's urgency as RMABs permeate into systems that impact human and wildlife outcomes. Code is available at https://github.com/google-research/socialgood/tree/equitable-rmab

==> 3_proofs_mathjax.tex <==
%%%%%%%%%%%%% Page 1
## Proof of Thm. 2
**Thm. 2.**
$L_g^0(\\cdot,b)$ is monotone increasing and concave in $b$.

**Proof.**

We drop the subscript $g$ for ease of notation. Let $\\boldsymbol{\\lambda}$ be the $H$-length vector of Lagrange multipliers $\\lambda^k$ for each timestep. Taking the derivative of $L^0$ with respect to $b$, we have

\\begin{equation*}\\tag{1}
\\frac{dL^0}{db} = H\\sum^{H-1}_{k=0}\\lambda^k
\\end{equation*}
Further, all $\\lambda_k\\ge 0$ following the Lagrangian relaxation of upper bound constraints in the *max* problem. So
\\begin{equation*}
\\frac{dL^0}{db} \\ge 0
\\end{equation*}
Thus $L^0(\\cdot,b)$ is monotone increasing in $b$. 

Moreover, the derivative of $L^0$ with respect to $\\boldsymbol{\\lambda}$ for each timestep is:

\\begin{align*}
&\\frac{dL}{d\\boldsymbol{\\lambda}} = \\tag{2}\\\\
&\\left[\\sum_{n=1}^{N}\\mathbb{E}[-a^0_{n}] + b, \\sum_{n=1}^{N}\\mathbb{E}[-a^1_{n}] + b,\\ldots,\\sum_{n=1}^{N}\\mathbb{E}[-a^{H-1}_{n}] + b\\right].
\\end{align*}

Note that $\\sum_{n=1}^{N}\\mathbb{E}[-a^k_n]$ is sum of the expected value of the cost of the actions over all $N$ arms at the timestep $k$, with respect to the optimal policy (derivative of the optimal value function) and the state transition probabilities. Setting Eq.~2 to 0 we get that:
\\begin{equation*}\\tag{3}
\\sum_{n=1}^{N}\\mathbb{E}[a^k_n] = b, \\hspace{2mm} \\forall k \\in [1,\\ldots,T].
\\end{equation*}
In other words, the optimal solution sets the Lagrange multipliers (effectively, "action charge multipliers") $\\boldsymbol{\\lambda}$ such that the optimal policy takes actions with sum total cost of $b$ in expectation at each timestep. This implies that as $b$ increases, the expected cost of actions taken by the optimal policy each round also increases. 

We now establish further properties of Eq.~1, by establishing how $\\boldsymbol{\\lambda}$ vary with $b$ at the optimal solution of $L^0$. To do so, we reason about whether $\\boldsymbol{\\lambda}$ must increase or decrease such that $\\sum_{n=1}^{N}\\mathbb{E}[a^k_n]$ would increase. 

We can observe from Eq.~4 in the main text that $\\boldsymbol{\\lambda}$ controls the cost of acting, and that the optimal relaxed arm value functions $V^k_n(\\cdot, \\boldsymbol{\\lambda})$ are piece-wise linear convex functions of $-\\boldsymbol{\\lambda}$ (max over piece-wise linear convex function is also piece-wise linear convex). This implies that, generally, as $\\boldsymbol{\\lambda}$ decreases, the policy will take actions with larger values of $a_{nj}^k$ on more arms. However, for this to be true for all values of $\\boldsymbol{\\lambda}$ is equivalent to Whittle's condition of indexability [Whittle, 1989], a common condition for restless bandit problems. Under this condition, decreasing $\\boldsymbol{\\lambda}$ implies increasing $\\sum_{n=1}^{N}\\mathbb{E}[a^k_n]$ and vice versa.

Hence, as $b$ increases, the values of $\\lambda^k$ decrease at the optimal solution for $L$. And thus, Eq.~1 is a decreasing function in $b$, implying that $L^0$ is concave in $b$.
\\end{proof}











%%%%%%%%%%% Page 2
## Proof of Thm. 3
**Thm. 3.**
$L_g^0(\\cdot,b) - V_g^0(\\cdot,b) < \\epsilon$ where $\\epsilon = (N-b)H$.

**Proof.**
Again we drop the subscript $g$ for ease of exposition. For this analysis, we assume arms have the same transition functions and start state $s_n^0$. 

Let the policy which never acts on a given arm be $\\underline{\\pi}\_n$. Let the policy which always acts on a given arm be $\\overline{\\pi}\_n$.

First, we establish that the Lagrangian bound is tight at $b=0$.

Observe Eq. 3 from the proof of Thm. 2. At $b=0$:

\\begin{equation*}
\\sum_{n=1}^{N}\\mathbb{E}[a^k_n] = 0, \\hspace{2mm} \\forall k \\in [1,\\ldots,T].
\\end{equation*}

Since $a^k_{nj} \\ge 0$ $\\forall n, j, k$, the optimal arm value functions in Eq. 4 of the main text $V^k_n(\\cdot, \\boldsymbol{\\lambda})$ must correspond to policies that always take actions with cost exactly $a^k_{nj} = 0$. This implies that the Lagrange bound gives the policy $\\underline{\\pi}\_n$ for all arms. This also implies that the values $\\lambda^k$ do not affect the solution, and thus the problem is decoupled, since only $\\lambda^k$ couples the individual arm value functions $V^k_n(\\cdot, \\lambda)$. Moreover, since $b=0$, the solution to Eq. 4, reduces to:


\\begin{align*}\\tag{4}
L^0(\\boldsymbol{s}^0,b=0) &= \\sum_{n=1}^{N}V_{n}^{0}(s_n^0, \\underline{\\pi}\_n) + b\\sum_{t=0}^H \\lambda^t \\\\
&= \\sum_{n=1}^{N}V_{n}^{0}(s_n^0, \\underline{\\pi}\_n)
\\end{align*}


where $V_{n}^{0}(s_n^0, \\underline{\\pi}\_n)$ is the value function of the policy $\\underline{\\pi}\_n$ for arm $n$ starting at time $0$ and state $s_n^0$.

Conversely, note that any policy at a given budget level $b$ is a lower bound on the un-relaxed value function $V^0(\\boldsymbol{s}^0,b)$. Let $\\underline{\\pi}$ be the trivial policy which never acts on any arms. Clearly the value function of $\\underline{\\pi}$ is also given by:

\\begin{equation*}\\tag{5}
\\underline{V}^0(\\boldsymbol{s}^0, \\underline{\\pi}) = \\underline{V}^0(\\boldsymbol{s}^0, b=0)  = \\sum_{n=1}^{N}V_{n}^{0}(s_n^0, \\underline{\\pi}\_n).
\\end{equation*}

Since $L^0$ upper bounds $V^0$, $\\underline{V}^0$ lower bounds $V^0$, and since $L^0(\\cdot,b=0) = \\underline{V}^0(\\cdot, b=0)$, the upper bound $L^0$ is tight at $b=0$.

Next, we establish that the Lagrangian bound is tight at $b=N$. Assume, without loss of generality, that $a^k_{nj} \\le 1$. Then Eq. 3 from the proof of Thm. 2 at $b=N$ gives:

\\begin{equation*}
\\sum_{n=1}^{N}\\mathbb{E}[a^k_n] = N, \\hspace{2mm} \\forall k \\in [1,\\ldots,T].
\\end{equation*}

In words, each $\\lambda^k$ should be set such that the optimal policy takes the most expensive action on every arm in expectation. This is achieved when the action charge multipliers $\\lambda^k = 0$ $\\forall k$. Alternatively, this can be interpreted as the shadow price of further relaxation of a constraint which is not tight. I.e., when $b=N$ and $a^k_{nj} \\le 1$, there is effectively no budget constraint. When all $\\lambda^k$ are 0, then the relaxed problem is again decoupled, since $\\lambda^k$ are the only terms that couple arms in the Lagrangian relaxation.

So for $b=N$, the solution to Eq. 4 reduces to:

\\begin{align*}\\tag{6}
L^0(\\boldsymbol{s}^0,b=N) &= \\sum_{n=1}^{N}V_{n}^{0}(s_n^0, \\overline{\\pi}\_n) + b\\sum_{t=0}^T \\lambda^t \\\\
&= \\sum_{n=1}^{N}V_{n}^{0}(s_n^0, \\overline{\\pi}\_n)
\\end{align*}

Conversely, let $\\overline{\\pi}$ be the policy which always takes the most expensive action on all arms. Clearly the value function of $\\overline{\\pi}$ is also given by:

\\begin{align*}\\tag{7}
\\underline{V}^0(s_n^0,\\overline{\\pi}) = \\underline{V}^0(s_n^0,b=N) = \\sum_{n=1}^{N}V_{n}^{0}(s_n^0, \\overline{\\pi}\_n)
\\end{align*}

Similarly, $L^0(\\cdot,b=N) = \\underline{V}^0(\\cdot, b=N)$, and so the upper bound $L^0$ is tight at $b=N$. Moreover, since $L^0(\\cdot,b)$ is monotone increasing (Thm. 2):

\\begin{align*}\\tag{9}
L^0(\\boldsymbol{s}^0,b) \\le \\sum_{n=1}^{N} V_{n}^{0}(s_n^0, \\overline{\\pi}\_n) \\hspace{2mm} \\text{ where } 0 \\le b \\le N
\\end{align*}

**Proof continued on on next page.**
















%%%%%%%%%%%% Page 3

### Proof 3 continued
Now we consider a lower bound on $V^0(\\boldsymbol{s},b)$, namely $\\underline{V}^0(\\boldsymbol{s}^0,b)$. It is convenient to analyze the value function of a policy which acts on the same $b$ arms each round, consisting of per-arm value functions $V_n(s^0_n, \\overline{\\pi}\_n)$ which act every round and $V_n(s^0_n, \\underline{\\pi}\_n)$ which never act:

\\begin{align*}\\tag{10}
\\underline{V}^0(\\boldsymbol{s}^0,b) = \\sum_{n=1}^b V_{n}^{0}(s_n^0, \\overline{\\pi}\_n) + \\sum_{n=b}^N V_{n}^{0}(s_n^0, \\underline{\\pi}\_n)
\\end{align*}

Then to bound the gap between $L^0$ and $V^0$, it is sufficient to bound the gap between $L^0$ and $\\underline{V}^0$. That is, $L^0(\\cdot,b) - V^0(\\cdot,b) = \\epsilon$, where:

\\begin{align*}\\tag{11}
\\epsilon &\\le \\sum_{n=1}^N V_{n}^{0}(s_n^0, \\overline{\\pi}\_n) - \\sum_{n=1}^{b}V_{n}^{0}(s_n^0, \\overline{\\pi}\_n) - \\sum_{n=b}^N V_{n}^{0}(s_n^0, \\underline{\\pi}\_n) \\\\
 &\\le \\sum_{n=b}^N V_{n}^{0}(s_n^0, \\overline{\\pi}\_n) - V_{n}^{0}(s_n^0, \\underline{\\pi}\_n) \\\\
 &\\le (N-b)H
\\end{align*}

Where the final step comes from assuming, without loss of generality, that all per-step rewards are between 0 and 1.
\\end{proof}


## Thm. 4 Proof.

**Thm. 4**
The following inequalities hold $\\hspace{1mm} \\forall g, \\hspace{1mm} \\forall a \\in M^{-1}(g), \\hspace{1mm} \\forall b$:

\\begin{equation*}\\tag{12}
v^a(b) \\le V_g(b) \\le |M^{-1}(g)| \\max_{c\\in M^{-1}(g)}v^c(b).
\\end{equation*}

**Proof.**
Recall that we define 
*arm-value functions*, namely, $v^a(b)$, which capture the value function of the single arm $a$, given budget $b$. These are in contrast to *group-value functions* $V_g(b)$ which are the value function of the optimal RMAB policy over all arms $a\\in|M^{-1}(g)|$ given per-round budget $b$. We define a composite function $h_g$ to characterize the relationship between the arm-value functions in a group $g$ and the group-value function of the group $g$.

Specifically, $h_g$ maps the set of all arm-value functions in a group $\\mathcal{A} = \\{v^a : a \\in M^{-1}(g)\\}$ to group-value functions $V_g$. E.g., if group $g$ has two arms $c$ and $d$, then $V_g(b) = h_g(\\{v^c, v^d\\})(b)$. We are interested in the relationship of $h_g$ and one of its input arm value functions $v^a$. 

First, we consider the lower bound on $h_g$.  Consider all sets $\\mathcal{A}$ such that $|\\mathcal{A}| > 2$. Similar, to the technique used in the proof of Thm. 3, we can consider the value of a specific sub-optimal policy to measure the lower bound. Specifically, the optimal value of $h_g(\\mathcal{A})(b) = V_g(b)$ is lower bounded by a policy which gives $b$ budget to just one of its arms and 0 to all others. Formally, we have:
\\begin{align*}\\tag{13}
h_g(\\mathcal{A})(b) &\\ge v^a(b) + \\sum_{i=1}^{|\\mathcal{A}|-1}v^{(\\mathcal{A} - \\{a\\})(i)}(0) \\hspace{2mm} \\forall a \\in \\mathcal{A} \\\\
&\\ge v^a(b) \\hspace{2mm} \\forall a \\in \\mathcal{A}
\\end{align*}

Then, we consider the upper bound. The results on the monotone increasing structure of $V_g(b)$ hold also for arm-value functions $v^a(b)$ (consider $V_g(b)$ with group size of 1). Since the composite function $h_g(\\mathcal{A})(b)$ causes a limited budget of $b$ to be shared across many arms, the composite function $h_g$ can be seen as reducing the *effective* budget of each individual $v^a$ included in the composite. Alternatively, we can show that $h_g$ gives functions that are upper bounded by composites of arm value functions that *do not* have to share budget. Formally:
\\begin{align*}\\tag{14}
h_g(\\mathcal{A})(b) &\\le \\sum_{a \\in \\mathcal{A}} v^a(1) \\hspace{3mm} \\text{always act on all arms} \\\\
&\\le \\sum_{a \\in \\mathcal{A}} v^a(b) \\hspace{2mm} \\forall b \\ge 1 \\\\
&\\le |\\mathcal{A}|\\max_{a}v^a(b).
\\end{align*}
This gives the proof and the key result that $h_g$ is a composite that scales more slowly in $b$ than the sum of its input functions. 
\\end{proof}


==> img/transition_diagram_dropout.tex <==
\begin{figure}
    \centering
    
\begin{tikzpicture}[node distance=2cm and 1cm,>=stealth',auto, every place/.style={draw,minimum size=2cm,text width=2cm,align=center,node distance=1cm}]
    \node [place] (S1) {$s_E=\textbf{\texttt{Maint.}}$\\\mbox{$s_C=\bm{C}$}\\$s_M=\bm{M}$};
    \node [place] (S2) [below=of S1] {$s_E=\textbf{\texttt{D.O.}}$\\\mbox{$s_C=\bm{C}$}\\$s_M=\bm{M}$};
    
    % Transitions within engaged
    \path[->] (S1) edge [bend left=30,dashed] node {$\bm{M}=[\texttt{Diseng.}, \texttt{Diseng.}]$} (S2);

       
\end{tikzpicture}

\caption{Construction of the transition from \textbf{\texttt{Maintenance}} state to \textbf{\texttt{Dropout}} state. The probability is only non-zero if the user was \texttt{Disengaged} for the previous two months, and does not receive an intervention this round, i.e., $a=\texttt{no call}$. \jon{to understand correctly, using this additional Memory, we dont need a linear interpolation and only instantiate transitions after 3 mo (noew 70\%)}}
\label{fig:transition_diagram_dropout}
\end{figure}
